Bang-Bang Control Of A Tail-less Morphing Wing Flight

Bats' dynamic morphing wings are known to be extremely high-dimensional, and they employ the combination of inertial dynamics and aerodynamics manipulations to showcase extremely agile maneuvers. Bats heavily rely on their highly flexible wings and are capable of dynamically morphing their wings to adjust aerodynamic and inertial forces applied to their wing and perform sharp banking turns. There are technical hardware and control challenges in copying the morphing wing flight capabilities of flying animals. This work is majorly focused on the modeling and control aspects of stable, tail-less, morphing wing flight. A classical control approach using bang-bang control is proposed to stabilize a bio-inspired morphing wing robot called Aerobat. Robot-environment interactions based on horseshoe vortex shedding and Wagner functions is derived to realistically evaluate the feasibility of the bang-bang control, which is then implemented on the robot in experiments to demonstrate first-time closed-loop stable flights of Aerobat.

==> unused.tex <==
\begin{figure}[t]
    \centering
    \vspace{0.1in}
    \includegraphics[width = \linewidth]{figures/plot_states.pdf}
    \caption{Body states.}
    \vspace{-0.1in}
    \label{fig:simulation_results_states}
\end{figure}

\begin{figure}[t]
    \centering
    \vspace{0.1in}
    \includegraphics[width = \linewidth]{figures/plot_thrusters.pdf}
    \caption{Thruster forces.}
    \vspace{-0.1in}
    \label{fig:simulation_results_thrusters}
\end{figure}
